Dallah: A Dialect-Aware Multimodal Large Language Model for Arabic

Recent advancements have significantly enhanced the capabilities of Multimodal Large Language Models (MLLMs) in generating and understanding image-to-text content. Despite these successes, progress is predominantly limited to English due to the scarcity of high quality multimodal resources in other languages. This limitation impedes the development of competitive models in languages such as Arabic. To alleviate this situation, we introduce an efficient Arabic multimodal assistant, dubbed Dallah, that utilizes an advanced language model based on LLaMA-2 to facilitate multimodal interactions. Dallah demonstrates state-of-the-art performance in Arabic MLLMs. Through fine-tuning six Arabic dialects, Dallah showcases its capability to handle complex dialectal interactions incorporating both textual and visual elements. The model excels in two benchmark tests: one evaluating its performance on Modern Standard Arabic (MSA) and another specifically designed to assess dialectal responses. Beyond its robust performance in multimodal interaction tasks, Dallah has the potential to pave the way for further development of dialect-aware Arabic MLLMs.

==> latex/eval_format.tex <==
\begin{figure}[H]
    \centering
    
      
  \centering
        \begin{tikzpicture}[node distance=12mm]
	\node (n1) [prompt] {
You are a specialized chatbot trained to evaluate the authenticity of Arabic
dialects.
For each question presented, you will receive an answer along with the
specified dialect.
Your task is to assess the authenticity of the dialect used in the answer on a
scale from 1 to 10, where 10 signifies perfect authenticity. And also to assess
the accuracy of the answer from the given context.
In your explanation of the score, mention the words that belong to the dialect
and those that lower the score because they are from Modern Standard Arabic
(MSA). Explain the relevance and completeness of the response.
Your explanation should be concise and clear and in a maximum of 50 words.
\includegraphics[width=\textwidth]{figs/eval_res_question.png}

% * قم باسترجاع المستندات ذات الصلة لاستعلام البحث على الويب بكلمة رئيسية قصيرة 
% والذي يطلب معلومات الطقس. 
% * ابحث عن المستندات التي تجيب على استفسار من نوع الأسئلة الشائعة حول تغذية  الأطفال.
% \textbf{Please adhere to the following guidelines:} \\
% Specify what the query is and what the desired documents are. Each retrieval task should cover a wide range of queries and not be too specific. Each of them must be in Modern Standard Arabic and related to the Arabic culture. Do not explain yourself or output anything else. Be creative! \\
}; 

\node (n3) [response, below=of n1]
	      {
       \includegraphics[width=\textwidth]{figs/eval.png}

          };
\draw [arrow] (n1) --  (n3);
\node[above left=0.15cm and -3.25cm of n3] (image) {\includegraphics[height=0.75cm]{figs/Untitled Diagram.drawio (6).png}};
\node[below= -0.25cm of image] {\scriptsize Evaluators};
\end{tikzpicture}
\caption{Methodology to evaluate dialect authenticity and content accuracy using model and human evaluators.}
\label{fig:prompt}
\end{figure}

==> sections/datasets_and_benchmarks.tex <==



==> sections/discussion.tex <==
\section{Discussion}
\label{discussion}
\todo[]{This section should be rephrased and aligned with previous section}
This study introduced \ourmodel, a multimodal large language model specifically designed for Arabic dialects. Our results demonstrated that \ourmodel significantly outperforms existing models in handling both MSA and six regional dialects.

Dallah\'s superior performance can be attributed to several key innovations. First, the novel data filtering method ensured that only high-quality, relevant multimodal datasets were used in the training process. This approach minimized the risk of error propagation due to translation inaccuracies and maximized the model's understanding of nuanced linguistic variations.

Moreover, the extensive fine-tuning across six major Arabic dialects, using limited but representative data, underscored the model\'s ability to adapt to diverse linguistic scenarios. This capability is critical in a region characterized by a rich tapestry of dialects, where linguistic diversity presents unique challenges for NLP systems.

However, the study also identified areas for future improvement. While Dallah excelled in dialect authenticity and content accuracy, variations in performance across different evaluators and dialects suggest that further refinement is needed. We have also shown that GPT4-Turbo and Command R+ are fairly competent at evaluating dialectal performance, with the latter being better at understanding dialects and accessing them. 

Additionally, the human evaluation highlighted the importance of incorporating cultural and linguistic nuances in model assessments. Future work could explore more sophisticated evaluation metrics or integrate additional human feedback to refine Dallah\'s performance further. 

